The influence of the Sun and Moon on the observation of very high energy gamma-ray sources using EAS arrays

With great advance of ground-based extensive air shower array, such as LHAASO and HAWC, many very high energy (VHE) gamma-ray sources have been discovered and are been monitored regardless of the day and the night. Hence, the Sun and Moon would have some compact on the observation of gamma-ray sources, which have not been taken into account in previous analysis. In this paper, the influence of the Sun and Moon on the observation of very high energy gamma-ray sources when they are near the line of sight of the Sun or Moon is estimated. The tracks of all the known VHE sources are scanned and several VHE sources are found to be very close to the line of sight of the Sun or Moon during some period. The absorption of very high energy gamma-ray by sunlight is estimated with detailed method and some usefully conclusions are achieved. The main influence is the block of the Sun and Moon on gamma-ray and their shadow on the cosmic ray background. The influence is investigated considering the detector angular resolution and some strategy on data analysis are proposed to avoid the underestimation of the gamma-ray emission.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

